OLALA: Object-Level Active Learning for Efficient Document Layout Annotation

Document images often have intricate layout structures, with numerous content regions (e.g. texts, figures, tables) densely arranged on each page. This makes the manual annotation of layout datasets expensive and inefficient. These characteristics also challenge existing active learning methods, as image-level scoring and selection suffer from the overexposure of common objects.Inspired by recent progresses in semi-supervised learning and self-training, we propose an Object-Level Active Learning framework for efficient document layout Annotation, OLALA. In this framework, only regions with the most ambiguous object predictions within an image are selected for annotators to label, optimizing the use of the annotation budget. For unselected predictions, the semi-automatic correction algorithm is proposed to identify certain errors based on prior knowledge of layout structures and rectifies them with minor supervision. Additionally, we carefully design a perturbation-based object scoring function for document images. It governs the object selection process via evaluating prediction ambiguities, and considers both the positions and categories of predicted layout objects. Extensive experiments show that OLALA can significantly boost model performance and improve annotation efficiency, given the same labeling budget. Code for this paper can be accessed via https://github.com/lolipopshock/detectron2_al.

==> tables/backup/performance-image-fixed.tex <==
\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{r|cc|cc}
        \toprule
        Datasets           & \multicolumn{2}{c|}{PubLayNet}     & \multicolumn{2}{c}{HJData}        \\
        \midrule
        Experiments        & AP                    & Total $I$/$O$  & AP                    & Total $I$/$O$ \\
        \midrule
        Image-Random       & 59.89                 & 1503/15980 & 63.42                 & 603/44156 \\
        \Olala-Random      & 57.96(-1.93)          & 1503/10228 & 65.72(+2.30)          & 603/29191 \\
        \midrule
        Image-Marginal     & 59.21                 & 1503/11848 & 69.04                 & 603/44251 \\
        \Olala-Marginal    & 53.33(-5.88)          & 1503/6829  & 65.84(-3.19)          & 603/30251 \\
        \Olala-Pertubation & \textbf{58.90(-0.31)} & 1503/\textbf{7496}  & \textbf{67.68(-1.36)} & 603/\textbf{28899} \\

        \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    %     \small
    %     \item[2,3] The \Olala-Random percentages are compared against Image-Random, and others are compared against Image-Marginal. 
    % \end{tablenotes}
    \end{threeparttable}
    }
    \caption{The final AP and number of total labeled images $I$ and objects $O$ when labeling the same number of images. \Olala maintains similar level of AP while requires labeling significantly less number of objects. Similar results are observed in PRImA and abbreviated to save space.}
    \label{table:performance-image-fixed}
\end{table}

==> tables/backup/performance-object-fixed.tex <==
% \begin{table}[]
%     \begin{tabular}{rcccccc}
%     Datasets          & \multicolumn{2}{c}{PubLayNet} & \multicolumn{2}{c}{HJData} & \multicolumn{2}{c}{PRImA} \\
%     Experiments       & AP             & Total I/O    & AP            & Total I/O  & AP            & Total I/O \\
%     Image-Random      & 60.73          & 2046/21430   & 69.82         & 709/51959  & 31.49         & 244/4799  \\
%     OLALA-Random      & 64.21+5.73\%   & 3187/21412   & 72.16+3.36\%  & 1105/51626 & 32.08+1.89\%  & 277/4785  \\
%     Image-Marginal    & 67.91          & 2465/21574   & 73.25         & 709/51937  & 30.99         & 243/4769  \\
%     OLALA-Marginal    & 69.23+1.93\%   & 3661/21467   & 71.48-2.42\%  & 1075/51804 & 32.85+6.00\%  & 306/4721  \\
%     OLALA-Pertubation & 69.13+1.79\%   & 3686/21430   & 73.40+0.20\%  & 1159/51656 & 33.87+9.30\%  & 286/4764 
%     \end{tabular}
% \end{table}


\begin{table*}[t]
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{r|cc|cc|cc}
        \toprule
        Datasets          & \multicolumn{2}{c|}{PubLayNet} & \multicolumn{2}{c|}{HJData} & \multicolumn{2}{c}{PRImA\tnote{1}} \\
        \midrule
        Experiments       & Final AP             & Total $I$/$O$    & Final AP            & Total $I$/$O$  & Final AP            & Total $I$/$O$ \\
        \midrule
        Image-Random      & 60.73        & 2046/21430   & 69.82         & 709/51959  & 31.49         & 244/4799  \\
        \Olala-Random      & \textbf{64.21(+3.48)}\tnote{2}     & 3187/21412   & \textbf{72.16(+2.34)}  & 1105/51626 & \textbf{32.08(+0.59)}  & 277/4785  \\
        \midrule
        Image-Marginal    & 67.91         & 2465/21574   & 73.25         & 709/51937  & 30.99         & 243/4769  \\
        \Olala-Marginal    & \textbf{69.23(+1.31)}\tnote{3}    & 3661/21467   & 71.48(-1.77)  & 1075/51804 & 32.85(+1.86)  & 306/4721  \\
        \Olala-Pertubation & 69.13(+1.21)   & 3686/21430   & \textbf{73.40(+0.15)}  & 1159/51656 & \textbf{33.87(+2.88)}  & 286/4764  \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \small
        \item[1] The figures in PRImA are the average from the 5 folds in cross validation to account for possible noise due to the small dataset size.
        \item[2,3] The \Olala-Random percentages are compared against Image-Random, and others are compared against Image-Marginal. 
    \end{tablenotes}
    \end{threeparttable}
    }
    \caption{The final AP and number of total labeled images $I$ and objects $O$ given the same object budget $m$. \Olala achieves strong performance improvements in model accuracy in all experiments, and creates datasets with considerably more images given the same labeling budget.}
    \label{table:performance-object-fixed}
\end{table*}

==> tables/performance.old.tex <==
\begin{table*}[t]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{r|lc|lc|lc}
        \toprule
        Dataset & \multicolumn{2}{c|}{PubLayNet}            & \multicolumn{2}{c|}{HJDataset}            & \multicolumn{2}{c}{PRImA\tnote{1}}  \\
        \midrule
        Exp   & Final AP                 & Labeled Images             & Final AP                 & Labeled Images           & Final AP                 & Labeled Images             \\
        \midrule
         Image-Random   & 60.73                    & 2046                       & 69.82                    & 709                      & 31.49                    & 244                        \\
         Image-Marginal & 67.91 (+11.84\%)         & 2465                       & 73.25 (+4.92\%)          & 709                      & 30.99 (-1.58\%)         & 243.6                      \\
        \Olala-Random   & 64.21 (+5.73\%)          & 3187 (+55.77\%)            & 72.16 (+3.36\%)          & 1105 (+55.85\%)          & 32.08 (+1.89\%)          & 277.80 (+13.85\%)          \\
        \Olala-Marginal & \textbf{69.23 (+14.00\%)}& 3661 (+78.93\%)            & 71.48 (+2.38\%)          & 1075 (+51.62\%)          & 32.85 (+4.33\%)          & \textbf{306.60 (+25.66\%)} \\
        \Olala-Perturbation  & 69.13 (+13.84\%)         & \textbf{3686 (+80.16\%)}   & \textbf{73.40 (+5.13\%)} & \textbf{1159 (+63.47\%)} & \textbf{33.87 (+7.57\%)} & 286.20 (+17.30\%)          \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \small
        \item[1] The figures in PRImA are the average from the 5 folds in cross validation to account for possible noise due to the small dataset size.
    \end{tablenotes}
    \end{threeparttable}
    }
    \caption{\textbf{The final AP and number of labeled images under different settings.} \Olala achieves strong performance improvements in model accuracy in all experiments, and creates datasets with more images given the same labeling budget.}
    \label{table:performance}
    \end{table*}
